An Empirical Study of DNNs Robustification Inefficacy in Protecting Visual Recommenders

Visual-based recommender systems (VRSs) enhance recommendation performance by integrating users' feedback with the visual features of product images extracted from a deep neural network (DNN). Recently, human-imperceptible images perturbations, defined \textit{adversarial attacks}, have been demonstrated to alter the VRSs recommendation performance, e.g., pushing/nuking category of products. However, since adversarial training techniques have proven to successfully robustify DNNs in preserving classification accuracy, to the best of our knowledge, two important questions have not been investigated yet: 1) How well can these defensive mechanisms protect the VRSs performance? 2) What are the reasons behind ineffective/effective defenses? To answer these questions, we define a set of defense and attack settings, as well as recommender models, to empirically investigate the efficacy of defensive mechanisms. The results indicate alarming risks in protecting a VRS through the DNN robustification. Our experiments shed light on the importance of visual features in very effective attack scenarios. Given the financial impact of VRSs on many companies, we believe this work might rise the need to investigate how to successfully protect visual-based recommenders. Source code and data are available at https://anonymous.4open.science/r/868f87ca-c8a4-41ba-9af9-20c41de33029/.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> Tables/notations.tex <==
\begin{table}[t]
    \centering
    \caption{Notations and their definition}

    \begin{tabular}{c c}
        \toprule
        \textbf{Notation} & \textbf{Definition} \\
        \bottomrule
         VRS & Visual-based Recommender System \\
         $\mathcal{U}$, $\mathcal{I}$, $\mathcal{P}$ & The set of users, items and feedback  \\
         UPM & User-item Preference-feedback Matrix \\
         $p_{ui}$ &  Feedback from user $u$ to item $i$ \\
         $\hat{p}_{ui}$ &  Predicted feedback from user $u$ to item $i$ \\

         \cmidrule(lr){1-2} 
         AML & Adversarial Machine Learning \\
         IFE & Image Feature Extractor \\
         $x_{i}$ & Image associated to item $i$ \\
         $x^*_{i}$ & Attacked image associated to item $i$ \\
         $y_i$ & True class for image $i$\\
         $C(x_i), \hat{y}_i$ & Predicted class for image $i$\\
         $C_s$ & Source class for a targeted attack\\
         $C_t$ & Target class for a targeted attack\\
         $\varphi_{i}$ & Features of image $i$ extracted with IFE\\
         $F(\cdot)$ & Clean feature extractor model function \\
         $\widetilde{F}(\cdot)$ & Defended feature extractor model function \\
         
        %  \cmidrule(lr){1-2} 
         
        %  $ASR$ & Attack Success Rate\\
        %  $FL$ & Feature Loss\\
        %  $LPIPS$ & Learned Perceptual Image Patch Similarity~\cite{DBLP:conf/cvpr/ZhangIESW18}\\
         
         \bottomrule
    \end{tabular}
    \label{table:notations}
\end{table}


==> Tables/success_rate.tex <==
\begin{table}[!t]
\caption{Average attacks success rate for each attack/defense combination.}
\centering
\scalebox{0.76}{
\begin{tabular}{llc|c|c}
\bottomrule
\multirow{2}{*}{\textbf{Dataset}} &  \multirow{2}{*}{\begin{tabular}[r]{@{}c@{}}\textbf{Adversarial}\\\textbf{Attack}\end{tabular}} & \multicolumn{ 3}{c}{\textbf{Image Feature Extractor}} \\ \cmidrule{3-5}
\multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{1}{c}{\textbf{Traditional}} & \multicolumn{1}{c}{\textbf{Adv. Train}} & \multicolumn{1}{c}{\textbf{Free Adv. Train}} \\  \bottomrule
\multirow{5}{*}{\begin{tabular}[r]{@{}c@{}}\texttt{Amazon}\\\texttt{Men}\end{tabular}} & FGSM ($\epsilon = 4$) & 65.45\% & 18.32\% & 15.18\% \\
\multicolumn{ 1}{c}{} & FGSM ($\epsilon = 8$) & 86.91\% & 23.56\% & 20.42\% \\ 
\multicolumn{ 1}{c}{} & PGD ($\epsilon = 4$) & 96.86\% & 18.32\% & 15.18\% \\ 
\multicolumn{ 1}{c}{} & PGD ($\epsilon = 8$) & 100.00\% & 24.08\% & 20.94\% \\ 
\multicolumn{ 1}{c}{} & C \& W & 89.01\% & 48.17\% & 42.41\% \\ \hline
\multirow{5}{*}{\begin{tabular}[r]{@{}c@{}}\texttt{Amazon}\\\texttt{Women}\end{tabular}} & FGSM ($\epsilon = 4$) & 17.70\% & 0.00\% & 0.00\% \\ 
\multicolumn{ 1}{c}{} & FGSM ($\epsilon = 8$) & 28.32\% & 2.65\% & 0.00\% \\ 
\multicolumn{ 1}{c}{} & PGD ($\epsilon = 4$) & 84.96\% & 0.00\% & 0.00\% \\ 
\multicolumn{ 1}{c}{} & PGD ($\epsilon = 8$) & 100.00\% & 3.54\% & 0.00\% \\ 
\multicolumn{ 1}{c}{} & C \& W & 89.38\% & 6.19\% & 6.19\% \\ \hline
\multirow{5}{*}{\begin{tabular}[r]{@{}c@{}}\texttt{Tradesy}\end{tabular}} & FGSM ($\epsilon = 4$) & 83.33\% & 43.33\% & 30.00\% \\ 
\multicolumn{ 1}{c}{} & FGSM ($\epsilon = 8$) & 93.33\% & 46.67\% & 46.67\% \\ 
\multicolumn{ 1}{c}{} & PGD ($\epsilon = 4$) & 100.00\% & 43.33\% & 30.00\% \\ 
\multicolumn{ 1}{c}{} & PGD ($\epsilon = 8$) & 100.00\% & 46.67\% & 46.67\% \\ 
\multicolumn{ 1}{c}{} & C \& W & 100.00\% & 80.00\% & 63.33\% \\ \bottomrule
\end{tabular}
}
\centering
\label{table:succes_rate}
\end{table}


==> samples/chr.tex <==
\begin{table*}[htbp]
\caption{}
\begin{center}

\resizebox{0.8\textwidth}{!}{
\begin{tabular}{|l|l|l|c|c|c|c|c|c|c|c|c|}
\hline
 \multirow{3}{*}{\textbf{Dataset}} &  \multirow{3}{*}{\textbf{MRS}} &  \multirow{3}{*}{\begin{tabular}[r]{@{}c@{}}\textbf{Adversarial}\\\textbf{Attack}\end{tabular}} & \multicolumn{ 9}{c|}{\textbf{Pre-trained Image Feature Extractor}} \\ \cline{ 4- 12}
\multicolumn{ 1}{|c|}{} & \multicolumn{ 1}{c|}{} & \multicolumn{ 1}{c|}{} & \multicolumn{ 3}{c|}{\textbf{Traditional}} & \multicolumn{ 3}{c|}{\textbf{Adv. Training}} & \multicolumn{ 3}{c|}{\textbf{Free Adv. Training}} \\ \cline{ 4- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & \multicolumn{ 1}{l|}{} & \multicolumn{1}{l|}{\chratventi} & \multicolumn{1}{l|}{\chratcinq} & \multicolumn{1}{l|}{\chratcento} & \multicolumn{1}{l|}{\chratventi} & \multicolumn{1}{l|}{\chratcinq} & \multicolumn{1}{l|}{\chratcento} & \multicolumn{1}{l|}{\chratventi} & \multicolumn{1}{l|}{\chratcinq} & \multicolumn{1}{l|}{\chratcento} \\ \hline
\multirow{18}{*}{\begin{tabular}[r]{@{}c@{}}\texttt{Amazon}\\\texttt{Men}\end{tabular}} & \multirow{6}{*}{VBPR} & Traditional & 0.6352 & 1.4931 & 3.0081 & 0.3028 & 0.8130 & 1.6928 & 0.3702 & 1.1547 & 2.3040 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & FGSM ($\epsilon=4$) & 0.5665 & 1.2607 & 2.4215 & 0.6029 & 1.4496 & 2.5943 & 0.5688 & 1.4924 & 2.5799 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & FGSM ($\epsilon=8$) & 0.6052 & 1.3498 & 2.6168 & 0.5879 & 1.4333 & 2.5520 & 0.5596 & 1.4433 & 2.5152 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & PGD ($\epsilon=4$) & 1.0936 & 2.6175 & 4.8287 & 0.6211 & 1.4763 & 2.6345 & 0.5778 & 1.5003 & 2.5856 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & PGD ($\epsilon=8$) & 1.5736 & 3.7285 & 6.6923 & 0.6247 & 1.4565 & 2.6011 & 0.6141 & 1.5768 & 2.7152 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & C \& W  & 0.5972 & 1.4003 & 2.6938 & 0.6652 & 1.4487 & 2.5865 & 0.6444 & 1.5641 & 2.6602 \\ \cline{ 2- 12}
\multicolumn{ 1}{|l|}{} & \multirow{6}{*}{AMR}& Natural & 0.3876 & 0.8587 & 1.8924 & 0.4924 & 1.1802 & 1.8572 & 0.1070 & 0.6255 & 1.1932 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{c|}{} & FGSM ($\epsilon=4$) & 0.3295 & 0.8282 & 1.7075 & 0.4332 & 1.1736 & 2.3897 & 0.4103 & 1.1595 & 2.2519 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & FGSM ($\epsilon=8$) & 0.3053 & 0.8668 & 1.8014 & 0.4318 & 1.1827 & 2.4155 & 0.4007 & 1.1250 & 2.2387 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & PGD ($\epsilon=4$) & 0.8064 & 1.9749 & 3.9621 & 0.4435 & 1.1756 & 2.4137 & 0.4173 & 1.1657 & 2.2810 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & PGD ($\epsilon=8$) & 2.1264 & 5.2984 & 9.6556 & 0.4323 & 1.1447 & 2.3144 & 0.3942 & 1.1386 & 2.2215 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & C \& W  & 0.3610 & 0.8171 & 1.7149 & 0.4293 & 1.1227 & 2.2999 & 0.4378 & 1.1623 & 2.2907 \\ \cline{ 2- 12}
\multicolumn{ 1}{|l|}{} & \multirow{6}{*}{LFM}& Natural & 0.4857 & 1.1959 & 2.5604 & 0.4003 & 0.9793 & 1.9482 & 0.3984 & 0.9791 & 1.9580 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{c|}{} & FGSM ($\epsilon=4$) & 0.5193 & 1.2670 & 2.5342 & 0.3811 & 0.9315 & 1.8372 & 0.3750 & 0.9324 & 1.8487 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & FGSM ($\epsilon=8$) & 0.5092 & 1.2693 & 2.5381 & 0.3715 & 0.9299 & 1.8458 & 0.3837 & 0.9281 & 1.8484 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & PGD ($\epsilon=4$) & 0.5147 & 1.2692 & 2.5417 & 0.3729 & 0.9187 & 1.8370 & 0.3735 & 0.9112 & 1.8209 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & PGD ($\epsilon=8$) & 0.5024 & 1.2672 & 2.5356 & 0.3765 & 0.9215 & 1.8438 & 0.3825 & 0.9367 & 1.8727 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & C \& W  & 0.5155 & 1.2573 & 2.5512 & 0.3765 & 0.9338 & 1.8484 & 0.3798 & 0.9428 & 1.8606 \\ 
\Xhline{2\arrayrulewidth}

\multirow{18}{*}{\begin{tabular}[r]{@{}c@{}}\texttt{Amazon}\\\texttt{Women}\end{tabular}}  & \multirow{6}{*}{VBPR} & Natural & 0.4377 & 1.2812 & 2.9440 & 0.5108 & 1.2390 & 2.5820 & 0.3417 & 0.9570 & 1.9529 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & FGSM ($\epsilon=4$) & 0.3860 & 1.0793 & 2.4827 & 0.6032 & 1.3813 & 2.3939 & 0.6088 & 1.1151 & 1.7664 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & FGSM ($\epsilon=8$) & 0.4057 & 1.2445 & 2.8671 & 0.6186 & 1.4160 & 2.4277 & 0.6313 & 1.1662 & 1.8784 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & PGD ($\epsilon=4$) & 0.9142 & 2.3673 & 4.6604 & 0.6309 & 1.4456 & 2.4965 & 0.6263 & 1.1165 & 1.7293 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & PGD ($\epsilon=8$) & 1.4462 & 3.4759 & 6.4732 & 0.6413 & 1.4674 & 2.5328 & 0.6139 & 1.1194 & 1.7740 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & C \& W  & 0.4147 & 1.2121 & 2.7236 & 0.6280 & 1.4277 & 2.4251 & 0.5729 & 1.1019 & 1.7287 \\ \cline{ 2- 12}
\multicolumn{ 1}{|l|}{} & \multirow{6}{*}{AMR}& Natural & 0.9449 & 2.0206 & 3.9123 & 0.8342 & 1.4602 & 2.5644 & 0.5063 & 0.7841 & 1.3467 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{c|}{} & FGSM ($\epsilon=4$) & 1.3173 & 2.4648 & 4.9918 & 0.7135 & 1.7675 & 3.0934 & 0.4565 & 1.0392 & 1.7776 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & FGSM ($\epsilon=8$) & 1.2814 & 2.2121 & 4.4605 & 0.7137 & 1.7595 & 3.0569 & 0.4429 & 1.0408 & 1.8077 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & PGD ($\epsilon=4$) & 1.1958 & 2.0161 & 3.7601 & 0.6473 & 1.7284 & 3.0676 & 0.4900 & 1.0750 & 1.8143 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & PGD ($\epsilon=8$) & 1.2377 & 2.6192 & 4.6613 & 0.6770 & 1.7451 & 3.0737 & 0.4445 & 1.0364 & 1.8057 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & C \& W  & 1.3012 & 2.2742 & 4.7353 & 0.7159 & 1.7976 & 3.1177 & 0.4977 & 1.0714 & 1.8397 \\ \cline{ 2- 12}
\multicolumn{ 1}{|l|}{} & \multirow{6}{*}{LFM}& Natural & 0.6771 & 1.6409 & 3.3157 & 0.4622 & 1.1589 & 2.3304 & 0.3186 & 0.7741 & 1.5253 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{c|}{} & FGSM ($\epsilon=4$) & 0.6816 & 1.6805 & 3.3592 & 0.4708 & 1.1550 & 2.2915 & 0.2985 & 0.7369 & 1.4731 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & FGSM ($\epsilon=8$) & 0.6880 & 1.6876 & 3.3612 & 0.4730 & 1.1593 & 2.3023 & 0.2985 & 0.7319 & 1.4645 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & PGD ($\epsilon=4$) & 0.6900 & 1.6920 & 3.3772 & 0.4737 & 1.1503 & 2.2853 & 0.3057 & 0.7451 & 1.4927 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & PGD ($\epsilon=8$) & 0.6727 & 1.6561 & 3.3107 & 0.4919 & 1.1811 & 2.3241 & 0.2988 & 0.7374 & 1.4645 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & C \& W  & 0.6746 & 1.6461 & 3.3484 & 0.4655 & 1.1409 & 2.2873 & 0.2844 & 0.7062 & 1.4315 \\

% \hline
\Xhline{2\arrayrulewidth}

\multirow{18}{*}{\tradesy} & \multirow{6}{*}{VBPR}& Natural & 0.4108 & 1.0721 & 2.1978 & 0.2973 & 0.7526 & 1.5461 & 0.3179 & 0.9602 & 2.0483 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & FGSM ($\epsilon=4$) & 0.5202 & 1.2273 & 2.4048 & 0.5055 & 0.9778 & 1.8721 & 0.5644 & 1.1905 & 2.3896 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & FGSM ($\epsilon=8$) & 0.7251 & 1.4667 & 2.5221 & 0.4807 & 0.9567 & 1.8092 & 0.4868 & 1.0908 & 2.3234 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & PGD ($\epsilon=4$) & 1.2552 & 2.2920 & 3.4304 & 0.4431 & 0.8885 & 1.7894 & 0.5217 & 1.1586 & 2.4060 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & PGD ($\epsilon=8$) & 1.6982 & 2.9039 & 3.9469 & 0.4726 & 0.9346 & 1.7366 & 0.5317 & 1.1580 & 2.4812 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & C \& W  & 0.4523 & 1.0561 & 2.1161 & 0.4766 & 0.9920 & 1.9127 & 0.5474 & 1.2309 & 2.5437 \\ \cline{ 2- 12}
\multicolumn{ 1}{|l|}{} & \multirow{6}{*}{AMR}& Natural & 0.3653 & 1.0573 & 2.1681 & 0.1626 & 0.5346 & 1.3232 & 0.2189 & 0.7609 & 1.9482 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{c|}{} & FGSM ($\epsilon=4$) & 0.4759 & 1.2386 & 2.3821 & 0.3587 & 0.8059 & 1.6598 & 0.4041 & 0.9674 & 2.0665 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & FGSM ($\epsilon=8$) & 0.5896 & 1.3448 & 2.4038 & 0.3512 & 0.7887 & 1.6168 & 0.3745 & 0.9132 & 2.0668 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & PGD ($\epsilon=4$) & 1.0393 & 1.9715 & 3.0360 & 0.3438 & 0.7686 & 1.6466 & 0.3635 & 0.8986 & 2.1294 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & PGD ($\epsilon=8$) & 1.6016 & 2.6768 & 3.5527 & 0.3494 & 0.7726 & 1.6347 & 0.3864 & 0.9416 & 2.1455 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & C \& W  & 0.4302 & 1.1161 & 2.2415 & 0.3577 & 0.8218 & 1.7366 & 0.3621 & 0.9178 & 2.1514 \\ \cline{ 2- 12}
\multicolumn{ 1}{|l|}{} & \multirow{6}{*}{LFM}& Natural & 0.3371 & 0.8935 & 1.8222 & 0.3579 & 0.8852 & 1.7799 & 0.4649 & 1.1398 & 2.2477 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{c|}{} & FGSM ($\epsilon=4$) & 0.3617 & 0.9098 & 1.8607 & 0.3744 & 0.9151 & 1.7940 & 0.5118 & 1.2292 & 2.4739 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & FGSM ($\epsilon=8$) & 0.3696 & 0.9232 & 1.8521 & 0.3822 & 0.9141 & 1.8185 & 0.5119 & 1.2271 & 2.4631 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & PGD ($\epsilon=4$) & 0.3603 & 0.9095 & 1.8183 & 0.3598 & 0.9024 & 1.7935 & 0.5081 & 1.2300 & 2.4742 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & PGD ($\epsilon=8$) & 0.4028 & 0.9811 & 1.9535 & 0.3741 & 0.9018 & 1.7943 & 0.5092 & 1.2295 & 2.4940 \\ \cline{ 3- 12}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 1}{l|}{} & C \& W  & 0.3750 & 0.9242 & 1.8841 & 0.3913 & 0.9356 & 1.8548 & 0.5116 & 1.2260 & 2.4667 \\ \hline
\end{tabular}

}
\end{center}
\label{}
\end{table*}


==> samples/old_sec3.tex <==
\section{PROPOSED FRAMEWORK: VAR}
\begin{figure*}[!t]
    \centering
    \includegraphics[width=\linewidth]{Figures/NewOverview.pdf}
    \caption{Overview of the proposed VAR framework for the evaluation of the consequences of adversarial attacks and defenses effects on a VRS. The adversary can perturb a product image, the Image Feature Extractor (IFE) composed by a traditional, or a defended, DNN extract the visual features, and the Visual Recommender System (VRS) gets in input the user-item preference matrix (UPM) and the extracted features and computes the top-$K$ recommendations.}
    \label{fig:var_architecture}
\end{figure*}
\flc{
In this section, we describe the proposed Visual Adversarial Recommendation (\var) framework to examine the application of adversarial attacks, and defenses, on visual-aware recommender models.
First, we define some preliminary concepts. Then we provide an overview of the \var components, including the adversary threat model, the feature extractor, and the visual recommender. Finally, we present new evaluation measures to quantify the effectiveness of the motivating scenario. 
}


\subsection{Preliminaries}
%\input{Tables/notations}
Here we underline some preliminary concepts and useful notation to formalize our work. 

% Table~\ref{table:notations} summarizes the key notations used throughout the rest of this paper.

\textbf{Recommendation Task.} We define the set of users, items and 0/1-valued preference feedback as $\mathcal{U}$, $\mathcal{I}$, and $\mathcal{P}$, where $|\mathcal{U}|$, $|\mathcal{I}|$, and $|\mathcal{S}|$ are the set sizes respectively. We reserve the use of $u$, $i$, and $p_{ui}$, to indicate a user of $\mathcal{U}$, an item in $\mathcal{I}$ and the feedback (e.g., a review) given by $u$ to $i$ saved in $\mathcal{P}$. Furthermore, we define the recommendation task as the action to suggest items that maximize, for each user, a utility function. We indicate with $\hat{p}_{ui}$ the predicted score learned from the recommender system (RS) upon historical preferences (represented as a user-item preference-feedback matrix (UPM)).

\textbf{Deep Neural Network.} Let $\mathcal{T}$ be a set of $M$ data samples $(x_i, y_i)$, $x_i \in \mathbb{R}^n$ and $y_i \in \mathbb{R}^m$. We define $F$ as a \textit{Deep Neural Network} model function trained on $\mathcal{T}$ to perform $m$-class classification, with $F(x_i) = \hat{y}_i$ the predicted probability distribution of $x_i$ belonging to each of the $m$ classes. Consequently, we calculate the class of the input $x_i$ as the index of $\hat{y}_i$ with maximum probability value, and represent it as $C(x_i)$. Moreover, assuming an $L$-layers DNN classifier, we adopt the notation $F_l(x_i)$, $l = \{0, 1, ..., L - 1\}$, as the output of the $l$-th layer of $F$ given the input $x_i$. 

% Let $\mathcal{T}$ be a set of $M$ data samples $(x_i, y_i)$, $x_i \in \mathbb{R}^n$ and $y_i \in \mathbb{R}^m$. We define a Neural Network (NN) as a function $F(\cdot)$ with parameters $\theta$, which, given the input $x_i$, returns $\hat{y}_i = F(x_i)$. In order to make $(x_i, \hat{y}_i)$ approximate the same distribution as $(x_i, y_i)$, $\theta$ is iteratively updated by minimizing a loss function $\mathcal{L}_F$, which depends on the task to solve:
% \begin{equation}
%     \underset{\theta}{\arg \min} \mathcal{L}_F(\theta, x_i, y_i)
% \end{equation}
% NNs consist of $L$ stacked layers, with $F_l(\cdot)$ being the output of the $l$-th layer and the input to the $(l + 1)$-th layer, $l = \{0, 1, ..., L - 2\}$. \textbf{Deep Neural Networks (DNNs)} are NNs with several stacked layers, commonly adopted to address complex AI tasks like image classification. In the remaining part of this paper, we will only refer to DNN models.  

% When a DNN is trained to solve an $m$-class classification task, $y_i$ represents the probability distribution of $x_i$ belonging to each of the $m$ possible classes. For this reason, $F_{L - 1}$ is commonly followed by a \textit{softmax} activation function so that the sum of probabilities over all classes sums to 1. We refer to $F_{L - 1}(x_i) = Z(x_i) = z_i$ as \textit{logits}, following the notation introduced in \cite{DBLP:conf/sp/PapernotM0JS16}. Hence, this holds true: $F(x_i) = \mathrm{softmax}(Z(x_i)) = \hat{y}_i$. Moreover, we define $F_t(x_i)$ as the probability of $x_i$ being classified as $t$. 

% Unless otherwise specified, for the sake of simplicity, we will refer to $y_i$ and $\hat{y}_i$ as the true and predicted classes for $x_i$ respectively (alternatively, $C(x_i)$ will also be adopted in place of $\hat{y}_i$). Additionally, in the context of this work, we will refer to $x_i$ only as an image, with height $h$, width $w$ and $c$ number of channels (e.g., $c = 3$ for an RGB image). 

\textbf{Adversarial Attack and Defense.} Given a DNN model function $F$ trained for classification, a pair of image/predicted class $(x_i, C(x_i))$, and following~\cite{DBLP:conf/sp/Carlini017}, we define an \textit{Adversarial attack} as the problem of finding the best value for a perturbation $\delta_i$ such that these three conditions are satisfied:
\begin{align}
    \label{eq:adversarial_attack}
    \begin{aligned}
    \text{minimize } &D(x_i, x_i + \delta_i) \\
     C(x_i + \delta_i) &\neq C(x_i)\\  
    x_i + \delta_i &\in [0, 1]^n
    \end{aligned}
\end{align}
where $D(\cdot)$ represents a \textit{distance metric} (e.g., $L_0$, $L_2$ and $L_{\infty}$ norms). The above definition states that (i) the attacked image $x_i^{*} = x_i + \delta_i$ must be visually similar to $x_i$, (ii) the predicted class for $x_i^{*}$ must be different from the original one and (iii) $x_i^{*}$ must stay within its original value range (i.e., $[0, 1]$ for 8-bit RGB images re-scaled by a factor 255). When $C(x_i^{*})$ is required to be generically different from $C(x_i)$, we say the attack is \textit{untargeted}. On the contrary, when $C(x_i^{*})$ is specifically required to be equal to a target class $C_t$, we say the attack is \textit{targeted}. 

Finally, we define a \textit{Defense} as the problem to find ways of limiting the impact of Adversarial attacks against a DNN. For instance, a common solution consists of training a more robust version of the original model function (we will refer to it as $\widetilde{F}$) which seeks to classify attacked images correctly:
\begin{equation}
    \widetilde{F}(x_i^{*}) = F(x_i) = C(x_i)
\end{equation}

% Given a DNN model function $F(\cdot)$ trained for classification, a pair of image/predicted class $(x_i, C(x_i))$, and inspired by~\cite{DBLP:conf/sp/Carlini017}, we define an \textit{Adversarial attack} as the problem of finding the best value for a perturbation $\delta_i$ such that these three conditions are satisfied:
% \begin{align}
%     \begin{aligned}
%     \text{minimize } &D(x_i, x_i + \delta_i) \\
%      C(x_i + \delta_i) &\neq C(x_i)\\  
%     x_i + \delta_i &\in [0, 1]^n
%     \end{aligned}
% \end{align}
% where $D(\cdot)$ represents a \textit{distance metric}. Common distance metrics in Adversarial attacks against images are $L_0$, $L_2$ and $L_{\infty}$ norms. The third condition states that the attacked image must stay within its original range of values (i.e., $[0, 1]$ for 8-bit RGB images re-scaled by a factor 255). 

% When changing the predicted class of the original image $x_i$ is the only important condition to meet, we say the Adversarial attack was \textbf{untargeted}. On the contrary, when the goal is to move the predicted class towards a specific \textit{target} class, we say the Adversarial attack was \textbf{targeted}. In the remaining sections of this paper, we will adopt the following notation: (i) $x^{*}_i = x_i + \delta_i$ to define an attacked image with perturbation $\delta_i$, (ii) $C_s$ as the source class for the Adversarial attack, and (iii) $C_t$ as the target class for the Adversarial attack.

% What is more, we define a \textbf{Defense} as the problem to find ways of limiting the impact of an Adversarial attacks against a DNN model. For instance, a common solution consists of training a more robust version of the original model function (we will refer to it as $\widetilde{F}(\cdot)$) which seeks to classify attacked images correctly:
% \begin{equation}
%     \widetilde{F}(x_i^{*}) = F(x_i) = C(x_i)
% \end{equation}

\subsection{Framework Overview}\label{sec:framework}
The proposed approach, shown in Figure~\ref{fig:var}, is composed by three main elements: the adversary (i.e., a malicious user), the image feature extractor (IFE), and the visual-based recommender model (VRS).  First, we describe the main characteristics of three aforementioned components. Then, we introduce a novel set of metrics to evaluate the recommendation performance at varying of recommenders, feature extractor, and adversarial attack strategies.  

\textbf{Adversary.}
In order to align with the AML literature, we follow the logical scheme described in~\cite{DBLP:journals/corr/abs-1902-06705}. \textbf{Adversary's goal} is to attack the Image Feature Extractor (IFE, see below) so that images of low-ranked categories of items are incorrectly classified as high-ranked ones. That is, the former will likely be recommended more (in average) than before. To this aim, not only is the adversary \textbf{aware} of all recommendation lists (used to choose the source and target classes), but she has also \textbf{perfect knowledge} of the IFE, i.e., its architecture, its trainable weights, and its output (white-box attack). Additionally, we suppose the adversary \textbf{can only perform} $L_{\infty}$ attacks, except for Carlini \& Wagner attack (see section \ref{subsec:adv_attacks}). Finally, in our scenario the adversary can \textbf{replace the original images} on the physical servers with the attacked one, which will eventually be exploited by the VRS to produce recommendations.     

\textbf{Image Feature Extractor (IFE).}
The input sample $x_{i}$ represents the $i$-th item photo the user sees on the e-commerce web page. Hence, the Image Feature Extractor (IFE) is a DNN pre-trained model ---on a classification task--- to extract high-level visual features from $x_i$. The actual extraction takes place at one of the final layer of the network, i.e., $F_e(x_i)$, with $e$ extraction layer. We define this layer output as $F_e(x_i) = \varphi_{i}$, and in similar works it usually is a $\mathcal{D}$-dimensional vector. In case of defense, IFE model function is simply replaced by $\widetilde{F}$. Indeed, feature extraction is a key operation in \var since it is the connection between the attack process and the consequent influence of the attack with respect to the recommendation task. 

\textbf{Visual-based Recommender System (VRS).}
The VRS is the component in the \var framework to address the recommendation task. The model accepts two inputs (i) the historical UPM, and (ii) the set of features of item images extracted from the IFE component, and produces sorted recommendation lists for each user in the system. The pure collaborative filtering source of data (i.e., the UPM), and the high-level latent representation of the multimedia content related to products catalog are integrated into the preference predictor of a VRS to unveil the visual aspects that arouse customer's preferences~\cite{DBLP:conf/aaai/HeM16}.
In the motivating example of \var, the influence on the performance of this component is the main objective of both the attacker, whose goal is to increase the recommendability of low-recommended categories of products by attacking the used IFE; and the defender, who tries to protect the recommendation performance. In this respect, the defender might act either on defending the IFE with the application of AML defense strategies (e.g., Adversarial Training~\cite{DBLP:journals/corr/GoodfellowSS14}), or adversarial regularizing the recommender model (e.g., AMR~\cite{8618394}).

\textbf{VAR Evaluation.}
To answer the research questions proposed in Section~\ref{sec:intro}, we need to perform three levels of analysis: (i) the effectiveness of the adversarial attack in misusing the classification performance of the DNN used to implement the IFE; (ii) the variation of the accuracy, and beyond-accuracy, recommendation performance, and (iii) the evaluation of the efficacy of attack strategies in \textit{pushing} the recommendability of the attacked category of items.  

We have identified several publications in AML on quantifying adversarial attacks success in corrupting the classification performance of an under attack classifiers~\cite{DBLP:journals/tnn/YuanHZL19}; as well as we have encountered a deep research literature on exploring several measures on the accuracy [XXX], and beyond accuracy [XXX], of RS. Conversely, the closest publications to this work are ~\cite{8618394, DSML20}. The authors of ~\cite{8618394} evaluate the effects of untargeted attacks on system accuracy metrics, i.e., \textit{Hit Ratio} (HR) and \textit{normalized Discounted Cumulative Gain} (nDCG); while the authors of ~\cite{DSML20} propose a modified version of HR, named Category Hit Ratio (\chr), that calculates the fraction of adversarially perturbed items in the top-$K$ recommendations. 

We define $I_{c} =  \{ i \in I | F(x_{i})=c\}$ as the set of items whose images are classified by the IFE in the $c$-class (i.e., the category of low recommended items) where $c \in \mathcal{C}$. We introduce $hit@K(u, k)$ as a 0/1-valued function that is $1$ when the item in the $k$-th position of the top-$K$ recommendation list of the user $u$ is in the set of attacked items not interacted by $u$. 
% ($\hat{i}_k \in I_c \setminus I^{+}_u $).
\begin{definition}[\categoryhitratio]
The \chr is defined as
\begin{equation}
    \label{eq:chr}
    \centering
    CHR@K = \frac{1}{|U|} \sum_{u \in U} \Big( \frac{1}{K} \sum_{k = 1}^{K} hit@K(u, k) \Big)
\end{equation}
\end{definition}

\walter{
Moreover, we propose a novel ranking-wise metric, named \textbf{Category normalized Discounted Cumulative Gain}, to measure the relevance of each recommended attacked item discounting its \textit{hit} in the top-$K$ recommendation list by a logarithmic factor that depends on its position.
\begin{definition}[Category n-DCG] 
We define \cndcg define as
\begin{equation}
    \label{eq:chr}
    \centering
    CnDCG@K = \frac{1}{|U|} \sum_{u \in U} \Bigg( 
    \frac{\sum_{k=1}^{K} \frac{hit@K(u, k)}{\log( k + 1)}} {\sum_{k=1}^{K} \frac{1}{\log( k + 1)}}
    \Bigg)
\end{equation}
\end{definition}
The \cndcg is ranged in a $[0, 1]$ interval, where value close to $1$ means that the attacked items are recommended in higher positions (e.g., the attack is effective). A logarithm with base 2 is commonly used to ensure all
positions are discounted}

==> samples/old_sec4.tex <==
\section{Experimental Setup}\label{sec:experiment}
In this section, we first introduce the three real-world recommender datasets in fashion domain. After that, we describe the adversarial attack strategies, details of the defense methods to make robust the feature extraction component, the baseline visual-based recommenders, and the experimental protocol used in the experimental evaluation of \var discussed in Section~\ref{sec:discussion}.

\subsection{Datasets}
\input{Tables/dataset}
In this section, we describe the three fashion-recommender datasets, which are drawn from two popular web platforms \textit{Amazon.com} and \textit{Tradesy.com}~\cite{DBLP:conf/sigir/McAuleyTSH15, DBLP:conf/www/HeM16}. 

\textbf{Amazon Men, Amazon Women.} The \amazonmen and \amazonwomen datasets contain user's ratings of "Clothing, Shoes and Jewelry" products category on the e-commerce catalog. After the download of the available images from the URLs published at \url{http://jmcauley.ucsd.edu/data/amazon/}, we have transformed any users' rating into an implicit 0/1-feedback.

\textbf{Tradesy.} The \tradesy dataset is a second-hand clothing selling social platform that contains implicit feedback (i.e., purchase histories, and desired products). Similar to \texttt{Amazon} dataset procedure, we have downloaded all available product pictures.

To reduce the degrading effects of cold-users, and items, we have applied different \textbf{\textit{k-core}} settings~\cite{DBLP:conf/www/HeM16}. In particular, we have chosen different \textbf{\textit{k}} values to explore different $sparsity$ dataset characteristic settings. Table~\ref{table:dataset_statistics} shows the dataset statistics as a result of the pre-processing steps described above. Datasets will be make available at publication time.


% , which have been demonstrated to impact the effect of attacks against collaborative recommenders~\cite{SIGIR2020}
% \dsml{
% \subsection{Adversarial Attacks}~\label{subsec:adv_attacks}
% We took into account two state-of-the-art adversarial attacks, i.e., Fast Gradient Sign Method (FGSM) and Projected Gradient Descent (PGD).
% }
% \dsml{
% \textbf{Fast Gradient Sign Method (FGSM)}~\cite{DBLP:journals/corr/GoodfellowSS14} focuses on the speed of the adversarial example generation. As a matter of fact, it generates an adversarial version of the attacked image in only one step. Given a clean input image $x$, a target class $t$, a model $F$ with parameters $\theta$, and a perturbation coefficient $\epsilon$, the targeted adversarial image $x^{*}$ is then
% \begin{equation}
%      x^{*} \xleftarrow{} x - \epsilon \cdot \mathrm{sign}(\nabla_x{\mathcal{L}_{F}}(\theta, x, t))
% \end{equation}
% where $\nabla_x\mathcal{L}_{F}(\theta, x, y)$ is the gradient of the $F$ loss function, and $\mathrm{sign(\cdot)}$ is the sign function.
% }
% \dsml{
% \textbf{Projected Gradient Descent (PGD)}~\cite{DBLP:conf/iclr/KurakinGB17a} iteratively applies FGSM, with a budget perturbation $\alpha$ (i.e., the step size) smaller than $\epsilon$. The attack algorithm works similarly to FGSM, but after each completed perturbation step, the temporary attacked image is clipped to remains in a $\epsilon$-neighborhood of the clean image $x$. The described approach is an extended and more effective version~\cite{DBLP:conf/icml/AthalyeC018} of Basic Iterative Method (BIM) proposed by Kurakin et al.~\cite{DBLP:conf/iclr/MadryMSTV18}. Indeed, PGD differs from BIM in the fact that PGD starts from a uniform random noise as the initial perturbation on the clean image $x$. The implemented version executes $10$ iterations. 
% For the implementation of both the algorithms, we adopted the Python library CleverHans~\cite{papernot2018cleverhans}. 
% }

\subsection{Adversarial Attacks and Defenses}~\label{subsec:adv_attacks} 
In this section we present all the adversarial attacks and defense techniques adopted in our work.

\subsubsection{Attacks}\label{subsubsection:attacks}
We explored three state-of-the-art adversarial attacks against images. 

\textbf{Fast Gradient Sign Method (FGSM)}~\cite{DBLP:journals/corr/GoodfellowSS14} is an $L_{\infty}$ norm optimized attack which produces an adversarial version of a given image in just one shot. 
% The sign of the gradient of the loss function (calculated with reference to $x$ and the target label class $C_t$) indicates the best direction to update the value of each pixel in $x$ so that it is classified as $C_t$. 
% A perturbation budget $\epsilon$ is set to variate the strength ---and the visibility--- of the attack. is set to make the attack undetectable. A final clipping to [a, b] range is performed. The attack is formalized as follows:
% \begin{equation}
%      x^{*} \xleftarrow{} \mathrm{clip_{[a, b]}}(x - \epsilon \cdot \mathrm{sign}(\nabla_x{\mathcal{L}_{F}}(\theta, x, C_t)))
% \end{equation}
% The value of a and b are set to the minimum and maximum pixel values of the original image respectively. 
A perturbation budget $\epsilon$ is set to modify the strength ---and consequently the visibility--- of the attack, i.e., higher $\epsilon$ values mean stronger attacks but also more evident visual artifacts. 
%is set to make the attack undetectable. 

\textbf{Projected Gradient Descent (PGD)}~\cite{DBLP:conf/iclr/MadryMSTV18} is an $L_{\infty}$ norm optimized attack which takes a uniform random noise as the starting perturbation budget and \textit{iteratively} applies FGSM with a continuously updated small perturbation $\alpha$ ---clipped within the $\epsilon$-ball--- until it gets to the final attacked image. 
% from produces the adversarial image $x^{*}$ through an iterative procedure. That is, instead of generating it in just one shot, it applies FGSM algorithm for a given number of iterations --for each iteration, a small perturbation budget $\alpha$ is adopted, and the produced perturbation is clipped within the $\epsilon$-ball-- until it gets to the final version of the attacked image. Differently from Kurakin et al.~\cite{DBLP:conf/iclr/MadryMSTV18}, PGD takes a uniform random noise as the starting perturbation budget, which helps increasing the robustness of the attack. 

\textbf{Carlini and Wagner attacks (C \& W)} are $L_0$, $L_2$ and $L_{\infty}$ norm optimized attacks proposed in~\cite{DBLP:conf/sp/Carlini017}. 
% able to break defensive techniques such as \textit{defensive distillation}~\cite{DBLP:conf/sp/PapernotM0JS16}. 
% Given an image $x$, a perturbation $\delta$ and a target class $t$, 
The authors re-formulate the traditional problem of finding an adversarial example (see again \ref{eq:adversarial_attack}) by replacing the distance metric with a suitably chosen \textit{objective function} which integrates a parameter $\kappa$, i.e., the \textit{confidence} of the attacked image being classified as $C_t$. An additional parameter $c$ sets the trade-off between optimizing the objective function and the classifier loss function. Finally, the overall problem is solved with \textit{gradient descent} and Adam as optimizer.

%$x^{*} \xleftarrow{} x + \delta$ as:

% \begin{equation}
%     \begin{aligned}
%         \text{minimize } \left\lVert \delta \right\rVert_p &+ c \cdot f(x + \delta) \\
%         \text{s.t. } x &+ \delta \in [0, 1]^n
%     \end{aligned}
% \end{equation}
% where $c$ is a constant to set a trade-off between giving more importance either to $x^{*}$ classification as $C_t$ or to $x^{*}$ being visually similar to the attacked image according to a distance metric, $p$ is the norm representing the distance metric, and $f(\cdot)$ is an objective function suitably chosen as:

% \begin{equation}
%     f(w) = \max (\underset{i \neq t}\max \{Z_i(w)\} - Z_t(w), -\kappa)
% \end{equation}
% with $\kappa$ defined as the \textit{confidence} of $w$ being classified as $t$. The parameter $c$ is found via \textit{binary search}. Finally, \textit{gradient descent} is run for a certain number of iterations, with Adam as optimizer. In the current work, we adopted the $L_2$ attack version. For a deeper understanding of the $L_0$ and $L_{\infty}$ attacks, please refer to the original paper. 

\subsubsection{Defenses} We also explored two defense strategies.

\textbf{Adversarial Training}~\cite{DBLP:journals/corr/GoodfellowSS14} consists of injecting adversarial samples into the training set to make the trained model robust to them. The major limitations of this idea are that it might increase the computational time to complete the training phase, and it is deeply dependent on the type of attack the adversarial images are created with. For instance, Madry \textit{et al.}~\cite{DBLP:conf/iclr/MadryMSTV18} generate PGD-based adversarial images to make the trained model robust against very strong attack methods. 

\textbf{Free Adversarial Training}~\cite{DBLP:conf/nips/ShafahiNG0DSDTG19} overcomes the computational cost of traditional adversarial training. For each minibatch, it computes the gradients with respect to the model parameters and with respect to the input image at the same time. Then, to simulate an iterative attack ---which would make the trained network more robust--- it keeps retraining on the same minibatch for $m$ times. The effect of this additional computational cost is mitigated by training the network for $N_E / m$ epochs, where $N_E$ is the number of epochs in a normal training. 

\subsection{Visual-based Recommender Models}~\label{subsec:recsys}
We study \var approach on three state-of-the-art baseline methods which utilize continuous visual features of items to improve the overall recommendation performance.

\textbf{Factorization Machine (FM)}~\cite{DBLP:conf/icdm/Rendle10} The Factorization Machine (FM) is a recommender model proposed by Rendle~\cite{DBLP:conf/icdm/Rendle10} to estimate the
user-item preference score with a factorization technique. For fair comparison with VBPR and AMR, we use the same BPR loss function to optimize personalized ranking, and we consider only user-item interactions and items features extracted from IFE component. 

\textbf{Visual Bayesian Personalized Ranking (VBPR)}~\cite{DBLP:conf/aaai/HeM16} is a typical matrix factorization CF model to learn user-item latent representation by optimizing a pairwise rank loss function. 
Given a user $u$, a not-interacted item $i$, the preference prediction score is defined as
\begin{equation}
    \hat{s}_{ui}= p_{u}^{T} q_{i} + \Theta_{u}^{T}(\mathbf{E} \varphi_{i}) + \beta_{ui}
    \label{eq:vbpr}
\end{equation}
where $p_{u} \in \mathbb{P}^{|U| \times \tau}$ and $q_{i} \in \mathbb{Q}^{|I| \times \tau}$ are latent vectors of user $u$ and item $i$, $\tau$ is the dimensionality of the latent space ($|\tau| << |U|, |I| $), $\theta_{u}$ is a $\pi$-dimensional vector to capture the visual interaction between $u$ and the projection $\varphi_i$ into a low-dimensional space through a $\pi \times \gamma$-kernel matrix $\mathbf{E}$, and $\beta_{ui}$ is the sum of the overall offset, user-item biases, and global visual bias.

\textbf{Adversarial Multimedia Recommendation (AMR)}~\cite{8618394} is an extension of VBPR that integrates the adversarial training procedure proposed by He \textit{et al.}~\cite{DBLP:conf/sigir/0001HDC18}, named \textit{adversarial regularization}, to construct a model increasingly robust to FGSM-based perturbations against image features. The score prediction function is the same of VBPR in Equation~\ref{eq:vbpr}. 


\subsection{Evaluation Metrics}

In addition to \chr and \cndcg metrics presented in Section~\ref{subsec:evaluation} to evaluate the effect of the adversarial attacks, we evaluate (i) the overall recommendation  performance, and (ii) the effects of the adversarial attacks both in misclassifying the classifier used for the feature extraction, and in perturbing the original image and its features.
Recommendation performance are evaluated with two well-known accuracy ranking-based metrics,  $Recall@K$, considers the fraction of recommended products in the top-$K$ recommendation that hit test items, and $nDCG@K$, increasingly discounts the hits by the $\log_2$ of the item positions in the list; and three beyond accuracy measures: the item coverage ($ICov@K$), the Gini index ($Gini@K$), and the expected free discovery ($EFD@K$). The evaluation of adversarial attacks (and defenses) performance is conducted through the Attack Success Rate ($ASR$), the Feature Loss ($FL$) calculated as the Mean Squared Error between the extracted image features before and after the attack, and the Learned Perceptual Image Patch Similarity ($LPIPS$), which evaluates the visual dissimilarity between two images (in our case, the original and attacked ones) by learning from several human judgments about original and modified images~\cite{DBLP:conf/cvpr/ZhangIESW18}. 

\subsection{Reproducibility}
Here, we provide reproducibility details of \var. The code and datasets are fully available at \url{http:\\mettere-il-link-anonimo}.

\textbf{Adversarial attacks.} All Adversarial attacks were implemented with the Python library CleverHans~\cite{papernot2018cleverhans}. For both FGSM and PGD we adopted $\epsilon = \{4, 8\}$ ---rescaled by 255--- since they are reasonable values to perturb the image efficiently without much visible artifacts. Then, for PGD's $\alpha$ parameter, we took the values of $\epsilon$ but re-scaled by 6, and the number of iterations was set to 10. 
As for C \& W attack, we run a 5-steps binary search to calculate $c$, starting from an initial value of $10^{-2}$. The confidence $\kappa$ was set to 0 and we adopted Adam optimizer with a learning rate of $5 \times 10^{-3}$ and a maximum number of iterations of 1000. 
% \daniele{mettiamo il discorso della normalizzazione con mean e std di ImageNet?}
% The library attack functions are written so to take min-max normalized images as input (e.g., within range $[0, 1]$), but our images were initially normalized with \imagenet mean and standard deviation. For this reason, we extended the original code to allow the algorithms to work with z-score normalized images. That is, we postponed the clipping operation in each attack only after a denormalization step. 
In order to actually reproduce the real-world scenario of a strong attacker targeting the IFE, we saved the attacked images in \texttt{tiff} format (i.e., a lossless compression), as it has been proven that lossy compression such as JPEG may affect the effectiveness of weaker attack methods~\cite{DBLP:conf/iclr/GuoRCM18}.

\textbf{Feature extraction and Defenses.} We used ResNet50~\cite{DBLP:conf/cvpr/HeZRS16} to extract high-level image features. From the PyTorch implementation, we set \texttt{AdaptiveAvgPool2d} as extraction layer, whose output is a $2048$-dimensional vector. In the non-defended scenario, we adopted ResNet50 pre-trained on \imagenet with traditional training. Conversely, when applying defense techniques, we adopted ResNet50 pre-trained on \imagenet with Adversarial Training and Free Adversarial Training. For the former, we used the pre-trained ResNet50 model online available~\footnote{\url{https://github.com/MadryLab/robustness}} with $\epsilon=4$. For the latter, we used a pre-trained model with $\epsilon=4$ and $m = 4$. Both trained models are available in the published GitHub repository.

\textbf{Recommenders.} We realize FM using the implementation available in LightFM's library~\cite{DBLP:conf/recsys/Kula15}. We trained the model for 100 epochs, and left all the parameters with the default values provided in the library. We have implemented both VBPR and AMR in \textit{Tensorflow}. We trained both the models for 4000 epochs following the training settings used in~\cite{8618394}. For each dataset we used the \textit{leave-one-out} training-test protocol putting in the test set the last time-aware user's interaction.

\textbf{Additional implementation details.} All experiments were performed using two Nvidia Tesla K80 GPUs with 12 GB memory.

\input{Tables/category}

